TheoremExplainAgent: Towards Video-based Multimodal Explanations for LLM Theorem Understanding

Understanding domain-specific theorems often requires more than just text-based reasoning; effective communication through structured visual explanations is crucial for deeper comprehension. While large language models (LLMs) demonstrate strong performance in text-based theorem reasoning, their ability to generate coherent and pedagogically meaningful visual explanations remains an open challenge. In this work, we introduce TheoremExplainAgent, an agentic approach for generating long-form theorem explanation videos (over 5 minutes) using Manim animations. To systematically evaluate multimodal theorem explanations, we propose TheoremExplainBench, a benchmark covering 240 theorems across multiple STEM disciplines, along with 5 automated evaluation metrics. Our results reveal that agentic planning is essential for generating detailed long-form videos, and the o3-mini agent achieves a success rate of 93.8% and an overall score of 0.77. However, our quantitative and qualitative studies show that most of the videos produced exhibit minor issues with visual element layout. Furthermore, multimodal explanations expose deeper reasoning flaws that text-based explanations fail to reveal, highlighting the importance of multimodal explanations.

==> tables.tex <==
\begin{table}[!t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|ccc}
 & Easy & Medium & Hard \\
\toprule
GPT-4o & 58/80 & 69/80 & 65/80  \\
Claude 3.5-Sonnet & TBC & TBC & TBC \\
Gemini 2.0-Flash & 14/80 & 17/80 & 10/80 \\
o3-mini & TBC & TBC & TBC \\
\bottomrule
\end{tabular} }
\caption{Agent Successful Rate in generating entire video.}
\label{tab:dataset_difficulty}
\end{table}


\begin{table}[!t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|cccc}
\toprule
 & Math & Phys & CS & Chem \\
\toprule
GPT-4o & TBC & TBC & TBC & TBC \\
Claude 3.5-Sonnet & TBC & TBC & TBC & TBC \\
Gemini 2.0-Flash & TBC & TBC & TBC & TBC \\
o3-mini & TBC & TBC & TBC & TBC \\
\bottomrule
\end{tabular} }
\caption{Agent Successful Rate in generating entire video for certain subjects.}
\label{tab:dataset_difficulty}
\end{table}


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/method_draft.png}
    \caption{Pipeline.}
    \vspace{-2ex}
    \label{fig:pipeline_design}
\end{figure}


\begin{table}[!t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|ccc}
\toprule
Agent & Easy & Medium & Hard \\
\toprule
GPT-4o & 41.3\% & 55.0\% & 37.5\% \\
Claude 3.5-Sonnet & 48.0\% & 58.0\% & 42.0\% \\
Gemini 2.0-Flash & 17.5\% & 21.3\% & 11.3\% \\
o3-mini (medium)& 83.8\% & 82.5\% & 80.0\% \\
\bottomrule
\end{tabular} }
\caption{Agent successful rate in generating entire video for different difficulty levels.}
\label{tab:dataset_difficulty}
\end{table}

\begin{table}[!t]
\centering
\scalebox{0.8}{
\begin{tabular}{l|cccc}
\toprule
Agent & Math & Phys & CS & Chem \\
\toprule
GPT-4o & 68.3\% & 40.0\% & 41.7\% & 28.3\% \\
Claude 3.5-Sonnet & 55.0\% & 40.0\% & 33.0\% & 20.0\% \\
Gemini 2.0-Flash & 26.7\% & 13.3\% & 15.0\% & 11.7\% \\
o3-mini (medium)& 81.7\% & 90.0\% & 88.3\% & 68.3\% \\
\bottomrule
\end{tabular} }
\caption{Agent successful rate in generating entire video for different STEM subjects.}
\label{tab:dataset_subject}
\end{table}

% Needs updating later
\begin{table*}[!t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|ccccc}
\toprule
Agent & Math & Physics & CompSci & Chem & Overall\\
\midrule
\multicolumn{6}{c}{Easy} \\
\midrule
TEA+GPT-4o & 75\% (96\%) & 55\% (90\%) & 65\% (94\%) & 50\% (91\%) & 61\% (93\%) \\
TEA+GPT-4o+RAG &  70\% (93\%) & 40\% (86\%) & 35\% (85\%) & 25\% (80\%) & 42\% (86\%) \\
TEA+Claude 3.5-Sonnet&  100 &  100 &  100 &  100 &  100 \\
TEA+Claude 3.5-Sonnet + RAG&  100 &  100 &  100 &  100 &  100 \\
TEA+Gemini 2.0 Flash &  35\% (81\%) & 10\% (70\%) & 25\% (76\%) & 10\% (76\%) & 20\% (76\%) \\
TEA+Gemini 2.0 Flash + RAG &  25\% (80\%) & 20\% (74\%) & 25\% (78\%) & 25\% (77\%) & 24\% (77\%) \\
TEA+o3-mini (medium) &  100\% (100\%) & 90\% (98\%) & 95\% (98\%) & 90\% (98\%) & 94\% (98\%) \\
TEA+o3-mini (medium) + RAG &  95\% (99\%) & 90\% (98\%) & 90\% (98\%) & 60\% (85\%) & 84\% (95\%) \\
\midrule
\multicolumn{6}{c}{Medium} \\
\midrule
TEA+GPT-4o & 60\% (91\%) & 55\% (93\%) & 75\% (96\%) & 40\% (88\%) & 57\% (92\%) \\
TEA+GPT-4o+RAG &  85\% (97\%) & 50\% (88\%) & 50\% (91\%) & 45\% (89\%) & 57\% (91\%) \\
TEA+Claude 3.5-Sonnet&  100 &  100 &  100 &  100 &  100 \\
TEA+Claude 3.5-Sonnet + RAG&  100 &  100 &  100 &  100 &  100 \\
TEA+Gemini 2.0 Flash &  15\% (79\%) & 10\% (59\%) & 20\% (78\%) & 0\% (54\%) & 11\% (67\%) \\
TEA+Gemini 2.0 Flash + RAG & 45\% (87\%) & 20\% (73\%) & 15\% (69\%) & 5\% (66\%) & 21\% (74\%) \\
TEA+o3-mini (medium) &  85\% (96\%) & 95\% (99\%) & 90\% (98\%) & 95\% (99\%) & 91\% (98\%) \\
TEA+o3-mini (medium) + RAG &  75\% (95\%) & 90\% (98\%) & 90\% (98\%) & 75\% (92\%) & 82\% (96\%) \\
\midrule
\multicolumn{6}{c}{Hard} \\
\midrule
TEA+GPT-4o & 50\% (90\%) & 55\% (91\%) & 35\% (86\%) & 45\% (91\%) & 46\% (89\%) \\
TEA+GPT-4o+RAG &  55\% (92\%) & 30\% (80\%) & 40\% (88\%) & 25\% (80\%) & 38\% (85\%) \\
TEA+Claude 3.5-Sonnet&  100 &  100 &  100 &  100 &  100 \\
TEA+Claude 3.5-Sonnet + RAG&  100 &  100 &  100 &  100 &  100 \\
TEA+Gemini 2.0 Flash &  0\% (67\%) & 5\% (56\%) & 20\% (77\%) & 25\% (81\%) & 12\% (71\%) \\
TEA+Gemini 2.0 Flash + RAG & 10\% (70\%) & 5\% (60\%) & 20\% (65\%) & 30\% (78\%) & 16\% (68\%) \\
TEA+o3-mini (medium) &  100\% (100\%) & 95\% (99\%) & 95\% (99\%) & 95\% (99\%) & 96\% (99\%) \\
TEA+o3-mini (medium) + RAG &  75\% (95\%) & 90\% (98\%) & 85\% (97\%) & 70\% (89\%) & 80\% (95\%) \\
\midrule
\multicolumn{6}{c}{Overall} \\
\midrule
TEA+GPT-4o & 62\% (92\%) & 55\% (91\%) & 58\% (92\%) & 45\% (90\%) & 55\% (91\%) \\
TEA+GPT-4o+RAG &  70\% (94\%) & 40\% (85\%) & 42\% (88\%) & 32\% (83\%) & 46\% (87\%) \\
TEA+Claude 3.5-Sonnet&  100 &  100 &  100 &  100 &  100 \\
TEA+Claude 3.5-Sonnet + RAG&  100 &  100 &  100 &  100 &  100 \\
TEA+Gemini 2.0 Flash &  17\% (76\%) & 8\% (61\%) & 22\% (77\%) & 12\% (70\%) & 15\% (71\%) \\
TEA+Gemini 2.0 Flash + RAG &  27\% (79\%) & 15\% (69\%) & 20\% (71\%) & 20\% (74\%) & 20\% (73\%) \\
TEA+o3-mini (medium) &  95\% (99\%) & 93\% (99\%) & 93\% (98\%) & 93\% (99\%) & 94\% (99\%) \\
TEA+o3-mini (medium) + RAG & 82\% (96\%) & 90\% (98\%) & 88\% (98\%) & 68\% (89\%) & 82\% (95\%) \\
\bottomrule
\end{tabular} }
\caption{Agent successful rate performances.}
\label{tab:succ_performances_app}
\end{table*}


% Latest
\begin{table*}[!t]
\centering
\scalebox{0.85}{
\begin{tabular}{l|ccc|cccc|c}
\toprule
Agent & Easy & Medium & Hard & Math & Phys & CS & Chem & Overall\\
\midrule
GPT-4o & 61.3\% & 57.5\% & 46.2\% & 61.7\% & 55.0\% & 58.3\% & 45.0\% & 55.0\%\\
GPT-4o + RAG & 42.5\% & 57.5\% & 37.5\% & 70.0\% & 40.0\% & 41.7\% & 31.7\% & 45.8\%\\
Claude 3.5-Sonnet v1 & 2.5\% & 1.2\% & 2.5\% & 1.7\% & 1.7\% & 1.7\% & 3.3\% & 2.1\% \\
Claude 3.5-Sonnet v1 + RAG & 18.8\% & 13.8\% & 11.2\% & 23.3\% & 10.0\% & 20.0\% & 5.0\% & 14.6\%\\
Gemini 2.0-Flash & 20.0\% & 11.2\% & 12.5\% & 16.7\% & 8.3\% & 21.7\% & 11.7\% & 14.6\%\\
Gemini 2.0-Flash + RAG & 23.8\% & 21.2\% & 16.2\% & 26.7\% & 15.0\% & 20.0\% & 20.0\% & 20.4\%\\
o3-mini (medium) & 93.8\% & 91.2\% & 96.2\% & 95.0\% & 93.3\% & 93.3\% & 93.3\% & 93.8\% \\
o3-mini (medium) + RAG & 83.8\% & 82.5\% & 80.0\% & 81.7\% & 90.0\% & 88.3\% & 68.3\% & 82.1\%\\
\bottomrule
\end{tabular} }
\caption{Agent success rate in generating complete videos across different difficulty levels and subjects.}
\label{tab:succ_diff_subject}
\end{table*}


\begin{table*}[!t]
\centering
\scalebox{0.85}{
\begin{tabular}{l|ccccc|c}
\toprule
Agent & Accuracy & Visual & Logical & Element & Visual & Overall \\
  & and Depth & Relevance & Flow & Layout & Consistency & Score \\
\midrule
GPT-4o & 0.79 &  0.79 &  0.89 &  0.59 &  0.87 & 0.78 \\
GPT-4o + RAG  &  0.75 &  0.77 &  0.88 &  0.57 &  0.86 &  0.76\\
Claude 3.5-Sonnet v1 &  0.75 &  0.87 &  0.88 &  0.57 &  0.92 &  0.79\\
Claude 3.5-Sonnet v1 + RAG&  0.67 &  0.79 &  0.69 &  0.65 &  0.87 &  0.71\\
Gemini 2.0 Flash  &  0.82 &  0.77 &  0.80 &  0.57 &  0.88 &  0.76\\
Gemini 2.0 Flash + RAG  &  0.79 &  0.75 &  0.84 &  0.58 &  0.87 &  0.76\\
o3-mini (medium) &  0.76 & 0.76 &  0.89 &  0.61 &  0.88 &  0.77 \\
o3-mini (medium) + RAG &  0.75 &  0.75 &  0.88 &  0.61 &  0.88 &  0.76\\
\midrule
Human-made Manim Videos &  0.80 &  0.81 &  0.70 &  0.73 &  0.87 &  0.77\\
\bottomrule
\end{tabular} }
\caption{Performance of our proposed metrics on successfully generated long-form videos by the agents.}
\label{tab:overall_performances}
\end{table*}

